Adversarial Machine Learning In Network Intrusion Detection Domain: A Systematic Review

Due to their massive success in various domains, deep learning techniques are increasingly used to design network intrusion detection solutions that detect and mitigate unknown and known attacks with high accuracy detection rates and minimal feature engineering. However, it has been found that deep learning models are vulnerable to data instances that can mislead the model to make incorrect classification decisions so-called (adversarial examples). Such vulnerability allows attackers to target NIDSs by adding small crafty perturbations to the malicious traffic to evade detection and disrupt the system's critical functionalities. The problem of deep adversarial learning has been extensively studied in the computer vision domain; however, it is still an area of open research in network security applications. Therefore, this survey explores the researches that employ different aspects of adversarial machine learning in the area of network intrusion detection in order to provide directions for potential solutions. First, the surveyed studies are categorized based on their contribution to generating adversarial examples, evaluating the robustness of ML-based NIDs towards adversarial examples, and defending these models against such attacks. Second, we highlight the characteristics identified in the surveyed research. Furthermore, we discuss the applicability of the existing generic adversarial attacks for the NIDS domain, the feasibility of launching the proposed attacks in real-world scenarios, and the limitations of the existing mitigation solutions.

==> 10.acknowledgmen.tex <==
The authors would like to thank...

==> 6.background.tex <==

\begin{comment}


This section provides brief background knowledge on the fundamentals of network intrusion detection, machine learning, deep learning, adversarial machine learning concepts, threat model, and the most common attack approaches. 
%==================================================%
\subsection{Network Intrusion Detection Fundamentals}
\textbf{Intrusion detection} is the process of dynamic monitoring and inspecting the events over a network or a system for suspicious behaviors that pose possible threats. An \textbf{intrusion detection system} is a hardware device or software application that performs such a task, and it can be mainly host-based or network-based. The \textbf{host-based IDS} monitors and logs malicious behaviors happening on a single host, such as unauthorized access attempts or files integrity violations. On the other hand, the \textbf{network-based IDS} monitors network traffic and inspects different network layers for suspicious activities such as flooding flow that indicates a DoS attack. The NIDS utilizes three major methodologies to detect malicious activities: signature-based, anomaly-based, and stateful protocol analysis. A \textbf{signature-based IDS} (i.e., misuse detection) detects intrusions by matching the network traffic to predefined patterns of known attacks with very low false alarms. The significant disadvantage of this approach is that it fails at detecting zero-day attacks.  An \textbf{anomaly-based IDS} (i.e., behavior-based) utilizes statistical, and machine learning approaches to detect anomalies and novel attacks by comparing the network packets to a profile of benign traffic in order to discover any deviation from the norm. Although it can detect zero-day attacks, it lacks accuracy as it tends to produce highly false positive alarms. A \textbf{stateful protocol analysis IDS}, (i.e., deep packet inspection) inspects the packets' content and tracks the state of used application protocols over the network. It compares the observed traffic to the normal activity of a protocol in order to discover deviations. 
%=========================================================%

\subsection{Adversarial Machine Learning Fundamentals}
~\citeauthor{szegedy2013intriguing}~\cite{szegedy2013intriguing} revealed for the first time that small but yet intentionally crafted perturbations (i.e., adversarial examples) added to the training inputs could lead the (NNs) models to misclassify, such as wrongly classifying "panda" to "gibbon". These examples were found to be transferable between models, which enable adversarial machine learning attacks in a black-box setting. The AEs are designed to fool a particular DL model can also be effective in misleading classification of different models; this property is called transferability. Such AEs that can transfer between different models are known as cross-modal AEs. Another form of transferability is cross-dataset, in which the AEs are generated by manipulating a particular dataset used to attack another model trained by a different dataset~\cite{ibitoye2019threat}.~\citeauthor{papernot2016limitations} ~\cite{papernot2016limitations} also discovered another form of AE's transferability that enables generated AEs based on a specific architecture of NNs to evade other different architectures and even other models trained by different ML algorithms. Furthermore, the AEs that are generated to deceive a specific NN can fool the same network even when it is trained by different datasets. In practice, the adversary utilizes these transfer-based attacks by using the outputs from the targeted model to train a substitute model and then crafting AEs for the surrogate model that are capable of transferring through the original model in a black-box setting~\cite{papernot2016transferability}. 


The ML algorithms depend on data for building models and performing classification tasks. These learned models can be misleading towards incorrect decisions with high confidence due to carefully crafted and manipulated perturbations added to legitimate inputs so-called \textbf{Adversarial Examples (AEs)}. In other words, an adversarial example is a data instance with tiny intentional feature perturbations that deceive the machine learning models and cause them to make a false classification. The adversarial examples undermine ML algorithms' fundamental assumption, which is data stationery (i.e., training and testing datasets have the same distribution). ML models assume that test data's distribution follows the training data, which is not the case in the real world case. Adversaries exploit this basic flawed assumption and use combinatorial optimization, local search, and convex programming to discover AEs that compromise the security of the models~\cite{usama2019generative}. Most approaches for generating the AEs add a calculated perturbation ($\gamma$) to a legitimate example ($x$) to generate a new version ($x^*$) (i.e., adversarial example) while minimizing the distance between the legitimate example ($x$) and the adversarial example ($x^*$), and shifting the prediction to the intended adversarial result. Adversarial machine learning (AML) attacks involve feeding these AEs p (i.e., perturbed inputs) to the model either at the training phase (poisoning attack) or inference phase (evasion attack) in order to force it into making wrong decisions. From the attacker's perspective, these examples are crafted to bypass detection by the models, perplex decision making, degrade their performance, probe them to gain information about the model parameters and training datasets. From the defender's perspective, they are utilized to conduct a vulnerability assessment and debugging for the models, evaluate their resilience to the noise, and increase their generalization abilities. Adversarial machine learning is an emerging research field that concerns with making ML models robust against adversarial attacks by assessing their vulnerabilities and accordingly designing the appropriate defensive mechanisms~\cite{huang2011adversarial}. 

%=========================================================%
\subsubsection{Adversarial Threat Model} provides an abstraction to profile the adversary based on aspects such as its capabilities, goals, knowledge, and strategies. A widely established taxonomy of adversarial attacks is proposed by~\citeauthor{huang2011adversarial}~\cite{huang2011adversarial}. It classifies attacks based on three main characteristics as follows:
\begin{itemize}
\item \textbf{Influence}, refers to the adversary's capabilities over the target model. Accordingly, that attacks can be causative attacks or exploratory attacks. \textbf{Causative attacks}, occur during the training time and aim to affect the process of learning the predictive function by the model, can also be called (poisoning attacks). \textbf{Exploratory attacks}, occur after the deployment of the model and may include probing the model in order to discover information  about its internal or its training dataset, such as (model stealing attacks)

\item \textbf{Security violation}, refers to the element of the CIA triad (i.e., the core foundation of information security) that the adversary compromises. It can be classified into integrity attacks, availability attacks, and privacy attacks. \textbf{Integrity attacks}, lead the model to classify the true positive data instances into false negative (e.g., an anomaly to normal). \textbf{Availability attacks}, lead the model to make wrong decisions, whether false positive or false negative, which cause it to be completely unusable. \textbf{Privacy attacks}, result in revealing information that violates the secrecy of the model or the privacy of its users. 

\item \textbf{Specificity}, refers to the span of the adversary's inputs that plans to be misclassified. It can be classified into targeted attacks or indiscriminate attacks. \textbf{Targeted attacks}, aim to force the model to misclassify a particular data instance or a small subset of data instances. \textbf{Indiscriminate attacks}, aim to force the model to misclassify a general class of data instances, such as classifying all the true positive data points into false negative. This attack degrades the model's reliability as its aim is to maximize prediction errors in general.%Huda you need to check of what you are saying is correct or not.

\end{itemize}
This taxonomy has been expanded to comprehensively cover definitive assumptions, which include the followings~\cite{carlini2019evaluating}:
\begin{itemize}
\item \textbf{Adversary knowledge}, refers to the extent of accessible knowledge about the model and its structural properties to the attacker. It can be categorized into white-box attacks, black-box attacks, and gray-box attacks. In \textbf{white-box attacks}, the adversary has complete knowledge about the model and its parameters (e.g., features, training dataset, algorithm, hyperparameters, in case of a NN that may include the model's architecture, weights, activation function, and the number of layers). Such knowledge is exactly what the creator of the model has, which in the majority of real-world scenarios is not feasible for the adversary to have. In \textbf{black-box attacks}, the adversary has no knowledge about the model or its parameters only knows the model's returned output (i.e., labels or confidence scores). This setting is commonly assumed for attacking online machine learning services. The adversarial attacks are mostly white-box; however, due to the transferability of AE, they can be used for black-box attacks, as well. In \textbf{gray-box attacks}, the adversary has constrained knowledge or limited access (e.g., access to the training dataset, access to the predicated classes, access to the predicted probabilities,  definite number of quires to the model). %================================================================%
\item \textbf{Strategy}: refers to the adversary's phases of actions for launching the attack, which can be one of the following: evasion attacks, poisoning attacks, or oracle attacks. \textbf{Evasion attacks}, so-called exploratory attacks, involve manipulating the inputs to deceive a previously trained model. In this attack, no influence over the training data is assumed. For instance, in a NIDS case, the attack payload is encoded to evade detection, compromising the targeted system. Additionally, the adversary may aim to provoke concept drift to the system causing continuous retraining and consequently degrading its performance.  It typically uses an optimization approach to find a small perturbation ($sigma$) that maximizes the loss function. Such an increase in loss function can be significant enough to cause the model to misclassify. \textbf{Poisoning attacks}, so-called causative attacks, involve corrupting the training data or model structure during training time in order to compromise the learning process, violate the built model's integrity, and degrade its performance in the deployment phase eventually. The adversary trains an anomaly-based NIDS with a labeled attack dataset as ground truth, causing the system's inability to detect cyber attacks. This type of attack can take one of the following forms data injection attacks, data manipulation attacks, or logic corruption attacks. In \textbf{data injection attacks}, the adversary has no access to the training dataset nor the model itself. However, the adversary can inject new perturbed inputs to intentionally manipulate training data's distribution. In \textbf{data manipulation attack}, the adversary has no access to the model but has access to the training dataset and manipulates it before it is used to train the model. It can take be either a label or input manipulation attack. In \textbf{label manipulation attacks}, the adversary has the ability to alter the labels of the training data only; for instance, a study has shown that flipping 40\% of class labels in the training dataset randomly is sufficient to degrade the performance of SVM classifiers~\cite{biggio2011support}. In \textbf{input manipulation attack}, the adversary has more power and can directly alter both of features and labels of the training dataset. In \textbf{logic corruption attacks}, the adversary has the ability to temper with the model itself and control it by altering its learning logic. 
\item \textbf{Oracle attack}, the adversary creates a substitute model that maintains most of the original model's functionality and designs attacks against it, to be later lunched against the original targeted model. Although this type of attack enables attacking the targeted system in a black-box setting, it suffers from a transferred loss as not all the AEs are able to transfer from one model to another. Therefore, a very large number of training instances are needed to train the substitute model to enhance the attack efficacy. It can be broken down into Extraction, Inference, and Inversion attacks. In \textbf{extraction attacks}, the adversary observes the model's outputs and class probabilities to infer internal information about the model, such as weights and parameters. \textbf{Inference attack}, the adversary may use a meta-classifier to collect useful information from other classifiers. Another form of this type of attack is \textbf{membership inference} in which the adversary queries using the target model in a black-box setting using a given data point to determine its presence in the training dataset and whether it belongs to the same distribution. The returned output from the model is a vector of probabilities that indicates whether the given data point pertains to a particular class. 
\textbf{Inversion attack}, reconstructs training data utilizing the given model parameters.  
\end{itemize}
%===============================================================%

Other researches extended the threat model further to cover the following:
\begin{itemize}
\item \textbf{Attack Mode}, it is commonly assumed in most of the related literature is that the adversary works on his own to achieve the attacks, \textbf{non-colluding attacks}. Another possible assumption is that multiple adversaries can cooperate to boost attacks' efficiency and hide their traces,  \textbf{colluding attacks}~\cite{pitropakis2019taxonomy}.
%================================================================%
\item \textbf{Attack Frequency}, refers to the times for an AE to be optimized. The attacks are categorized into one-time or iterative attacks based on the frequency of optimizing or updating the generated AEs. \textbf{One-time attacks} optimize the generated AEs one-time without any iteration. On the other hand, \textbf{iterative attacks} update AE multiple times. For a real-time attack, adversaries should choose a one-time attack instead of an iterative attack. Iterative updating result in better optimized AEs that overcome one-shot attacks; however, this approach is computationally expensive and require a greater extent of interactions with the targeted model (i.e., more queries)~\cite{yuan2019adversarial}.
%================================================================%
\end{itemize}
%&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&%
\subsubsection{Perturbation} adversarial examples are intended to be close as possible to the original examples. Therefore, introducing tiny perturbations is the fundamental premise for generating them. Three aspects to analyze the introduced perturbation: perturbation limitation, perturbation scope, and perturbation measurement~\cite{yuan2019adversarial}. 
%================================================================%
\begin{itemize}
    \item \textbf{Perturbation limitation}
    \begin{itemize}
        \item \textbf{Optimized perturbation}, define perturbation as the target of the optimization problem and aim for minimizing the introduced perturbation as much as possible.
        \item \textbf{Constraint perturbation}, define perturbation as the constraint of the optimization problem and demand it to be small enough.
    \end{itemize}
    \item \textbf{Perturbation scope}
        \begin{itemize}
        \item \textbf{Individual attacks}, craft distinct perturbations for each clean instance of the inputs. 
        \item \textbf{Universal attacks}, craft a general perturbation for the entire dataset, and this general perturbation is applicable to any clean input. Most of the existing adversarial techniques create the perturbations individually. Universal perturbations facilitate deploying adversarial examples in the real world. In such a case, the adversary does not need to amend the perturbation when the input changes.
    \end{itemize}
    \item \textbf{Perturbation measurement}
    \begin{itemize}
        \item \textbf{$l_p$} measures introduced perturbations by $p$-norm distance~\cite{yuan2019adversarial}. There are three $l_p$ distance metrics in the literature $l_0$, $l_2$, and $l_\infty$. \textbf{$l_0$} counts the number of features to be perturbed. \textbf{$l_2$} measures the Euclidean distance between the original and adversarial example. \textbf{$l_\infty$} denotes maximum magnitude of perturbation added to each feature. 
        \item Psychometric perceptual adversarial similarity score (PASS) is a metric for quantifying adversarial images. 
    \end{itemize}
\end{itemize}
%=========================================================%
\begin{figure*}[tp]
%\begin{adjustbox}{varwidth=\textwidth,margin=0 {\abovecaptionskip} 0 0, frame=0.50pt }
\includegraphics[width=\textwidth]{images/taxonomy.pdf}
%\end{adjustbox}
\caption{Threat Model of Adversarial Attacks}
\label{graph2}
\centering
\end{figure*}
%&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&

\subsubsection{Adversarial Attacks Algorithms}
Adversarial examples are used to attack machine learning models at training time (poisoning attacks) or at inference time (evasion attacks). To recall, white-box attacks can be launched when the adversary has access to the model gradients such as model weights. On the other hand, the in black-box attacks the adversary almost knows nothing about the targeted model and depends on the returned outputs to tweak the perturbations. White attacks are more powerful than the black-box ones as they succeed in crafting AEs that target the victim model with minimal effort and time and do not rely on attacks' transferability. The robustness of AEs generation techniques depends on their ability to produce AEs that are as close as possible to the original examples.  In the section below, the most commonly utilized AEs generation approaches in the literature are explained briefly and summarized in table~\ref{table:Summary of most common generic adversarial examples generation techniques}.
%================================================================%

\citeauthor{szegedy2013intriguing} \cite{szegedy2013intriguing} introduced \textbf{Broyden-Fletcher-Goldfarb-Shanno (L-BFGS)} technique to generate adversarial images using box-constrained limited memory approximation to minimize the added perturbations. ~\citeauthor{goodfellow2014explaining}~\cite{goodfellow2014explaining} presented the \textbf{Fast Gradient Sign Method (FGSM)} in order to reduce high computational cost of (L-BFGS). This method adds flat perturbations to each feature of the example. Due to its relatively computing cost, FGSM is one of the famous techniques for crafting AEs. However, it perturbs every feature of the example, making it applicable to some domains where features are changeable and unconstraint.~\citeauthor{kurakin2016adversarial} ~\cite{kurakin2016adversarial} proposed \textbf{Basic Iteration method (BIM)} which executes multiple iterations of FGSM with small steps to minimize the introduced perturbations. Although BIM is slower than FGSM, it results in crafting more subtle and powerful AEs.~\citeauthor{papernot2016limitations} ~\cite{papernot2016limitations} presented \textbf{Jacobian based Saliency Map Attack (JSMA)} which adds flat perturbations iteratively to produce AEs with high effectiveness and less distortion degree. It perturbs a few features as it looks for features that, with little change applied to it, would make large variations that lead to misclassification. However, it is slower than FGSM due to its computational cost as it is an iterative approach.~\citeauthor{moosavi2016deepfool} ~\cite{moosavi2016deepfool} introduced \textbf{Deepfool} which generates generalizable and transferable AEs.~\citeauthor{carlini2017towards}~\cite{carlini2017towards} proposed \textbf{Carlini and Wagner (CW)} which is similar to (L-BFGS) method but uses different objective functions and without box-constraints. The produced examples by this method can defeat some defensive techniques such as network distillation.~\citeauthor{xiao2018generating}~\cite{xiao2018generating} proposed utilizing \textbf{Generative Adversarial Network (GAN)} to craft AEs. A GAN consists of two neural networks, one generates the AEs, and the other tries to distinguish between the original and adversarial examples. Although it can produce different examples than those in the training dataset, training such a network is computationally intensive and can be unstable. ~\citeauthor{chen2017zoo}~\cite{chen2017zoo} proposed \textbf{Zeroth order optimization (ZOO)} an optimization-based method that estimates the gradient and hessian in a black-box setting by querying the targeted model with individual altered features each time. This method quires the victim model at each step to estimate the gradient; hence, it requires many quires to generate successful adversarial examples.
%================================================================%

\end{comment}

==> 8.defensemechanisms.tex <==
There are some defensive mechanisms proposed to defend DNNs against adversarial examples. The first defensive mechanisms were introduced by~\citeauthor{barreno2006can}~\cite{barreno2006can} and broadly include: Randomization, Regularization, and Information hiding. ~\citeauthor{yuan2019adversarial}~\cite{yuan2019adversarial} generally categorized countermeasures into \textbf{Reactive} that discover AEs after DNNs are trained, and \textbf{Proactive} that enhance  DNNs' resistance against AEs before they are being attacked. ~\citeauthor{ibitoye2019threat}~\cite{ibitoye2019threat} classified defense approaches based on attacker strategy. For poisoning attacks that occur during the training time, the defense approaches may include data sanitization, data encryption, and statistical robustness. In data sanitization, the cleanliness of the inputs is insured by rejecting the examples that may inititae negative impacts of the model. Meanwhile, for evasion attacks that occur during inference time, the defense approaches are adversarial training, differential privacy, and homomorphic encryption. Differential privacy utilizes randomiaztion approaches to protect the data during the training and testing stages. In homomorphic encryption, the model directly processes encrypted inputs. The most common used methods include~\cite{zhang2020tiki}: Adversarial Training~\cite{tramer2017ensemble}, Adversarial Detecting \& Rejecting~\cite{lu2017safetynet}, Network Distillation~\cite{papernot2016distillation}, Network Verification~\cite{katz2017reluplex}, Classifier Robustifying~\cite{abbasi2017robustness}, Input Reconstruction~\cite{samangouei2018defense}, Ensemble learning~\cite{yuan2019adversarial}. In this section, some of proposed defensive methods are briefly described. 

%==========================================================%
\textbf{Adversarial training} involves injecting AEs (e.g., malicious perturbed inputs) to the original dataset during the training phase, such that the deployed model can then resist better against the AEs. This method is useful only when the AEs are crafted based on the original model, and it is not resilient to black-box attacks when the examples are generated on a locally trained substitute model~\cite{chakraborty2018adversarial}. Furthermore, it can be bypassed by a two-step attack, where random perturbations are added firstly to the instance, followed by other perturbations performed by another classical attack. Additionally, the obtained robustness against AEs by this approach depends on the strength of utilized AEs during the adversarial training. For instance, a model is trained with FGSM-based AEs will have robustness against non-iterative attacks, but not against Projected Gradient Descent (PGD) attacks~\cite{vahakainu2020iot}. PGD-based adversarial training can provide the most robust protection against advanced powerful attacks; therefore, it is considered to be the state-of-the-art defensive mechanism. However, its costly computations degrade its potentiality to be used as an effective defense method. \textbf{Adversarial noise reduction}, in domains such as image processing and time-series data (e.g., weather and sensors readings) that suffer from different kinds of noise, the noise reduction techniques have shown the potentiality to mitigate AEs, such as utilizing stacked denoising autoencoders for that purpose~\cite{moosavi2018divide}. \textbf{Ensemble learning} (i.e., majority voting ensemble) uses a voting approach that combines the predictions of multiple pre-trained models to build a stronger one that is more robust and less susceptible to the AEs. \textbf{Network distillation} involves training a neural network (i.e., student) to learn knowledge from a pre-trained complex network (i.e., teacher). Hence, the student network will have better generalization capabilities and more resistance to the AEs. \textbf{Network verification} employs an additional model to detect the AEs before they are fed into the model for classification. \textbf{Adversarial Query Detection} works based on the concept that black-box attack approaches depend on querying the targeted model continuously and adjusting the added perturbations each time based on the received feedback to bypass the victim detector~\cite{zhang2020tiki}. The added perturbations in each attempt tend to be slightly small in such a way that the substance of the original input is not changed; thus, they result in highly similar queries for the same attack attempt. Such intrinsic similarities between the queries can be utilized to detect adversarial evasion attacks. \textbf{Classifier robustifying} utilizes different techniques such as ensembling to enhance the robustness of the original model. \textbf{Input Reconstruction} involves restoring the original inputs in order to reduce the effectiveness of the malicious perturbations. \textbf{Gradient masking}, as most of the adversarial attacks are gradient-based, this approach aims at modifying the machine learning model to obscure the gradient from adversaries. \textbf{Feature reduction}, showed its potentiality to mitigate the risks of evasion attacks~\cite{bhagoji2017dimensionality}. \textbf{Detecting adversarial examples}, utilizes different approaches and concepts to detect the adversarial examples, such as probability divergence, an auxiliary network of the original networks.  \textbf{Designing an effective ML algorthim}, a secure version of SVM called Sec-SVM, was introduced to protect the classifier from evasion attacks~\cite{demontis2017yes}. \textbf{Statistical testing}, can be used as a detection approach to distinguish between the authentic and adversarial examples as the adversarial ones are not drawn from the same distribution of the original dataset~\cite{grosse2017statistical}. \textbf{Robust optimization}, involves techniques that aim to smooth the decision boundaries of ML algorithms, hence reducing the impact of AEs~\cite{russu2016secure}. \textbf{Feature selection}, suggests training the model with a subset of features that the adversary cannot manipulate. Although such an approach may prevent some evasion attacks, the detection rates are degraded as a result of feature removal. 

%==========================================================%
\begin{comment}
A summary of presented defensive mechanisms along with their strengthens and weaknesses is shown in table \ref{table:Summary of adversarial ML attacks defense}. 
%\begin{table}[htbp]
\begin{table*}[t]
\centering
%\footnotesize 
\setlength{\tymin}{60pt} % not so narrow columns
% use \RaggedRight instead of \raggedright
%\let\raggedright\RaggedRight

\begin{tabulary}{\textwidth}{@{}|L|L|L|L|L|L|@{}}
%\toprule
\hline
\textbf{Mechanism} &
\textbf{Type} &
  \textbf{Description} &
  \textbf{Strengths} &
  \textbf{Weaknesses} &
  \textbf{Improvements} \\
%\midrule
\hline
Adversarial training & Proactive & injects AEs into the training dataset to boost model's robustness towards AEs. It utilizes AEs that are crafted by  generic AEs generation techniques. &
      low proliferative potential, not diffusive & - It is an adversarial attack-based defence technique. 
- The trained model can't generalize over AEs are generated by other attacks.
- \textcolor{red}{It can be evaded by indiscriminate perturbation from other models} . & Adversarial Training with Domain Adaptation (ATDA) method.~\cite{song2018improving}\\ \hline

Network distillation~\cite{papernot2016distillation} & & Description & it can be effective towards unknown threats; dynamic approach requires less human intervention; & With attaining high computation power and proper fine-tuning can be exploited using reverse engineering; vulnerable to poisoning attacks where the malicious inputs are injected into the preliminary training dataset; & Improvements\\ \hline
Noise reduction & type & Description & Strengths & Weaknesses & Improvements\\ \hline
Model Voting Ensembling & Proactive & trains a set of classifiers so-called (an ensemble of classifiers) and combines their predictions on unseen instances using a voting mechanism in order to produce improved classification results.  & Model gradient-estimation based attacks can be hindered as the voting approach induces the integral model to be non-differentiable; Crafting AEs that are able to simultaneously bypass all the models is more difficult than compromising an individual model; it doesn't require retraining to the original models therefore it's easy to implement;   & Weaknesses & Improvements\\ \hline
Adversarial Query Detection & Reactive & detects the querying process of the black-box attack, and prevents the attack form succeeding by blocking the attacker's IP address. & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
Mechanism & Type & Description & Strengths & Weaknesses & Improvements\\ \hline
%\bottomrule
%\hline
\end{tabulary}
\caption{Summary of adversarial ML attacks defense}
\label{table:Summary of adversarial ML attacks defense}
\end{table*}
\end{comment}



==> NewPapers.tex <==
~\cite{pacheco2021adversarial} 

==> images/neuralnetwork.tex <==
    \begin{neuralnetwork}[height=4]
        \newcommand{\x}[2]{$x_#2$}
        \newcommand{\y}[2]{$\hat{y}_#2$}
        \newcommand{\hfirst}[2]{\small $h^{(1)}_#2$}
        \newcommand{\hsecond}[2]{\small $h^{(2)}_#2$}
        \inputlayer[count=3, bias=true, title=Input\\layer, text=\x]
        \hiddenlayer[count=4, bias=false, title=Hidden\\layer 1, text=\hfirst] \linklayers
        \hiddenlayer[count=3, bias=false, title=Hidden\\layer 2, text=\hsecond] \linklayers
        %\hiddenlayer[count=3, bias=false, title=Hidden\\layer 44, text=\hsecond] \linklayers
        \outputlayer[count=2, title=Output\\layer, text=\y] \linklayers
    \end{neuralnetwork}

==> removed.tex <==
\subsection{Machine Learning Fundamentals}

\textbf{Machine learning} empowers computers to discover how to accomplish tasks without being explicitly programmed by learning from a provided dataset to solve the problem at hand. Machine learning encompasses various algorithms that can be mainly categorized according to their approach, application, and depth.    
\subsubsection{Machine Learning Approaches}
\begin{itemize}
\item \textbf{Supervised learning}, requires a labeled training dataset that consists of data instances and class labels pairs to learn a mapping function that maps an input ($x$) to the output ($y$). 
\item \textbf{Unsupervised learning}, no labels are provided in the training dataset, leaving the algorithm independently captures the hidden patterns and structures a compact internal representation of the data inputs. 
\item \textbf{Semi-Supervised learning}, represents centermost between supervised and unsupervised learning. It integrates a small amount of labeled data instances with many unlabeled ones for training in cases where a fully-labeled training is not readily available, or obtaining such a dataset is difficult, expensive, time-consuming, and demanding domain expertise.  
\item \textbf{Reinforcement learning}, does not require an initial training dataset; alternatively, the agent collects the data by interacting with its environment and optimizes the decision process towards a goal by learning from the consequences of its actions. Both reinforcement learning and supervised learning use mapping between the inputs and outputs. Supervised learning needs correct pairs of input and output to accomplish the task, while reinforcement learning employs rewards and punishments as indications for positive and negative actions.
\item \textbf{Ensemble Learning}, uses a combination of multiple learning models to achieve an overall performance that is better than what can be attained by using any single model. It can increase the accuracy and stability of learning models by reducing the errors that result from variance, bias, and noise.  
\end{itemize}
\subsubsection{Machine Learning Tasks}
Based on the approach and nature of available data, machine learning algorithms are used to build models that can achieve one of these most common tasks:
\begin{itemize}
    \item \textbf{Classification}, learns a predictive function from a pre-labeled dataset that can assign a class label for an unseen data instance. It approximates a mapping function ($f$) from labeled input instances ($X$) to discrete output classes ($y$). 
    \item \textbf{Clustering}, discovers hidden patterns in feature space of unlabeled inputs and groups these points based on similarities or distance measures into unknown classes (i.e., clusters).  
    \item \textbf{Dimensionality Reduction}, transfers a dataset from a high-dimensional space into a compact low-dimensional space while maintaining the significant characteristics of the original dataset as much as possible.  
    \item \textbf{Regression}, learns a predictive function by examining the relationship between a set of variables predictors (independent) and responses (independent) and estimates a continuous-value outcome for a given observation, accordingly. 
    \item \textbf{Association Rule Learning}, uses metrics of interestingness to identify strong rules that relate between the antecedent ($X$) and the consequence of rule ($Y$).  
    %\item \textbf{Generative Modeling},
\end{itemize}
\subsubsection{Machine Learning Depth}
\begin{itemize}
    \item \textbf{Shallow Learning}, encompasses the techniques of conventional machine learning that do not utilize multiple layers or hidden connections. 
    \item \textbf{Deep Learning}, uses multiple layers of nodes in the artificial neural network that can extract a high-level representation of feature from raw inputs. 
\end{itemize}

\subsection{Deep Learning Fundamentals}
\textbf{Deep learning} is a subfield of machine learning based on artificial neural networks. \textbf{Neural networks} are biologically inspired by the structure of the human brain and imitate its behavior to solve complex data-driven problems. An ANN consists of layers of perceptrons known as neurons that form the network's core processing units. A NN consists mainly of an input layer that acquires the inputs, an output layer that predicts the final result, and one or multiple hidden layers (i.e., deep neural network) in between that perform the complex computations. The neurons in one layer are connected to the other neurons in the next layer through links. These links are initially assigned random numerical values termed weights. Each neuron multiplies its inputs with their corresponding weights and adds its associated numerical value called the bias. This weighted sum is passed through a non-linear function called the activation function, which acts as a threshold to determine whether the neuron is activated or not. When a neuron is activated, its output is transmitted to the neurons in the next layer; this process of propagating the data through the network is called forward-propagation. In the output layer, the neuron has the highest activation value determines the final output in the form of a probability of prediction. The network is trained by adjusting its weights using the back-propagation algorithm in order to minimize error in prediction (i.e., the difference between the actual output and predicted output). Intuitively, the weights that contribute to correct predictions are increased, and the ones that contribute to wrong predictions are decreased. The network continually performs iterative cycles of forward-propagation and back-propagation to adjust the weights using multiple inputs until it succeeds in making correct predictions for most of the inputs. Figure~\ref{structure of a neuron in a neural network} shows an illustration for a neuron in a NN\footnote{Source: becominghuman.ai}.
\begin{figure}[!htp]
 \includegraphics[width=\columnwidth]{images/structure of a neuron in a neural network.png}
\caption{structure of a neuron in a neural network}
\label{structure of a neuron in a neural network}
\centering
\end{figure}

Deep neural networks (DNN) are advanced enough to perform feature engineering using raw inputs independently. The use of multiple hidden layers enables extracting features and finding latent structures in unprocessed and unlabeled inputs. The figure~\ref{Structure of deep neural network} graphically illustrates the architecture of a typical DNN composed of multiple layers (at least two hidden layers) of neurons. Each layer learns to transform its multidimensional inputs into a more compact and abstract representation. Therefore, the network can be entirely viewed as a highly complex non-linear mapping function that converts high-dimensional inputs into a lower-dimensional space.
 

\begin{figure}[h]
%\input{images/neuralnetwork.tex}
    \scalebox{0.92}{\input{images/neuralnetwork.tex}}
    \caption{Structure of deep neural network}
\label{Structure of deep neural network}
\end{figure}
